Code Prediction by Feeding Trees to Transformers

We advance the state-of-the-art in the accuracy of code prediction (next token prediction) used in autocomplete systems. First, we report that using the recently proposed Transformer architecture even out-of-the-box outperforms previous neural and non-neural systems for code prediction. We then show that by making the Transformer architecture aware of the syntactic structure of code, we further increase the margin by which a Transformer-based system outperforms previous systems. With this, it outperforms the accuracy of an RNN-based system (similar to Hellendoorn et al. 2018) by 18.3%, the Deep3 system (Raychev et al 2016) by 14.1%, and an adaptation of Code2Seq (Alon et al., 2018) for code prediction by 14.4%. We present in the paper several ways of communicating the code structure to the Transformer, which is fundamentally built for processing sequence data. We provide a comprehensive experimental evaluation of our proposal, along with alternative design choices, on a standard Python dataset, as well as on a Facebook internal Python corpus. Our code and data preparation pipeline will be available in open source.

==> main.tex <==
% %%
% %% This is file `sample-sigconf.tex',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% samples.dtx  (with options: `sigconf')
% %%
% %% IMPORTANT NOTICE:
% %%
% %% For the copyright see the source file.
% %%
% %% Any modified versions of this file must be renamed
% %% with new filenames distinct from sample-sigconf.tex.
% %%
% %% For distribution of the original source see the terms
% %% for copying and modification in the file samples.dtx.
% %%
% %% This generated file may be distributed as long as the
% %% original source files, as listed above, are part of the
% %% same distribution. (The sources need not necessarily be
% %% in the same archive or directory.)
% %%
% %% The first command in your LaTeX source must be the \documentclass command.
% % \documentclass[format=acmsmall, review=true, anonymous=true]{acmart}
% \documentclass[format=acmsmall, nonacm]{acmart}
% \usepackage{listings}
% \usepackage{diagbox}
% \usepackage{fancybox}
% \usepackage{natbib}
% \setcitestyle{numbers}


% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% % \setcopyright{acmcopyright}
% % \copyrightyear{2018}
% % \acmYear{2018}
% % \acmDOI{10.1145/1122445.1122456}

% %% These commands are for a PROCEEDINGS abstract or paper.
% % \acmConference[ESEC/FSE 2020]{
% %   The 28th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering
% %   }{8 - 13 November, 2020}{Sacramento, California, United States}
% % \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
% %   June 03--05, 2018, Woodstock, NY}
% % \acmPrice{15.00}
% % \acmISBN{978-1-4503-XXXX-X/18/06}


% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}

% \input{preamble} % our packages and defs
% %%
% %% end of the preamble, start of the body of the document source.
% \begin{document}

% %%
% %% The "title" command has an optional parameter,
% %% allowing the author to define a "short title" to be used in page headers.
% \title{Code Prediction by Feeding Trees to Transformers}

% %%
% %% The "author" command and its associated commands are used to define
% %% the authors and their affiliations.
% %% Of note is the shared affiliation of the first two authors, and the
% %% "authornote" and "authornotemark" commands
% %% used to denote shared contribution to the research.
% \author{Seohyun Kim}
% \authornote{Both authors contributed equally to this research.}
% \affiliation{%
%   \institution{Facebook Inc.}
%   \country{U.S.A.}
% }
% \email{skim131@fb.com}

% \author{Jinman Zhao}
% \authornotemark[1]
% \affiliation{%
%   \institution{University of Wisconsin-Madison}
%   \country{U.S.A.}
% }
% \email{jz@cs.wisc.edu}

% \author{Yuchi Tian}
% \affiliation{%
%   \institution{Columbia University}
%   \country{U.S.A.}
% }
% \email{yuchi.tian@columbia.edu}

% \author{Satish Chandra}
% \affiliation{%
%   \institution{Facebook Inc.}
%   \country{U.S.A.}
% }
% \email{schandra@acm.org}

% %%
% %% By default, the full list of authors will be used in the page
% %% headers. Often, this list is too long, and will overlap
% %% other information printed in the page headers. This command allows
% %% the author to define a more concise list
% %% of authors' names for this purpose.
% % \renewcommand{\shortauthors}{Kim, et al.}

% %%
% %% The abstract is a short summary of the work to be presented in the
% %% article.
% \begin{abstract}

% We advance the state-of-the-art in the accuracy of code prediction
% (next token prediction) used in autocomplete systems.  First, we report that using the recently proposed Transformer architecture even out-of-the-box outperforms previous neural and non-neural systems for code prediction.  We then show that by making the Transformer architecture aware of the syntactic structure of code, we further increase the margin by which a Transformer-based system
% outperforms previous systems.  With this, it outperforms the accuracy of an RNN-based system (similar to Hellendoorn et al.~\citeyear{hellendoorn2017deep}) by 18.3\%, the \ETH system~\cite{raychev2016probabilistic-deep3-eth-dt} by 14.1\%, and 
% an adaptation of \CSeq~\cite{alon2018codeseq} for code prediction by 14.4\%.

% We present in the paper several ways of communicating the code structure to the Transformer, which is fundamentally built for processing sequence data. 
% We provide a comprehensive experimental evaluation of our proposal, along with alternative design choices, on a standard Python dataset, as well as on a Facebook internal Python corpus.
% Our code and data preparation pipeline will be available in open source.
  
% \end{abstract}

% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%
% % \begin{CCSXML}
% % <ccs2012>
% %   <concept>
% %       <concept_id>10010147.10010257.10010293.10010294</concept_id>
% %       <concept_desc>Computing methodologies~Neural networks</concept_desc>
% %       <concept_significance>500</concept_significance>
% %       </concept>
% %   <concept>
% %       <concept_id>10010147.10010257.10010258.10010260</concept_id>
% %       <concept_desc>Computing methodologies~Unsupervised learning</concept_desc>
% %       <concept_significance>300</concept_significance>
% %       </concept>
% %   <concept>
% %       <concept_id>10011007.10011074.10011092.10011782</concept_id>
% %       <concept_desc>Software and its engineering~Automatic programming</concept_desc>
% %       <concept_significance>500</concept_significance>
% %       </concept>
% %  </ccs2012>
% % \end{CCSXML}

% % \ccsdesc[500]{Computing methodologies~Neural networks}
% % \ccsdesc[300]{Computing methodologies~Unsupervised learning}
% % \ccsdesc[500]{Software and its engineering~Automatic programming}

% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% % \keywords{code completion, deep learning, transformer models}

% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% % \begin{teaserfigure}
% %   \includegraphics[width=\textwidth]{sampleteaser}
% %   \caption{Seattle Mariners at Spring Training, 2010.}
% %   \Description{Enjoying the baseball game from the third-base
% %   seats. Ichiro Suzuki preparing to bat.}
% %   \label{fig:teaser}
% % \end{teaserfigure}

% %%
% %% This command processes the author and affiliation and title
% %% information and builds the first part of the formatted document.
% \maketitle

% \input{sec/introduction}


% \input{sec/models}

% \input{sec/model-tree}

% \input{sec/backgroundtree}

% \input{sec/implementation}

% \input{sec/evaluation}

% \input{sec/inspection}

% \input{sec/threats}

% %\input{sec/related-works}

% \input{sec/future-work}


% %%
% %% The acknowledgments section is defined using the "acks" environment
% %% (and NOT an unnumbered section). This ensures the proper
% %% identification of the section in the article metadata, and the
% %% consistent spelling of the heading.
% % \begin{acks}
% % To Robert, for the bagels and explaining CMYK and color spaces.
% % \end{acks}

% %%
% %% The next two lines define the bibliography style to be used, and
% %% the bibliography file.
% \bibliographystyle{plainnat}
% \bibliography{main}

% %%
% %% If your work has an appendix, this is the place to put it.
% \appendix
% \input{sec/appendix}

% \end{document}
% \endinput
% %%
% %% End of file `sample-sigconf.tex'.


==> tab/top-aggr-ud-paths.tex <==
% This is a generated file. Do not manually modify. See <filename>.py instead.
\begin{table}[]
    \centering
    \begin{tabular}{l | c}
    \hline
    UD path & Score \\
    \hline
    \code{2U} & 0.236 \\
\code{U2D} & 0.151 \\
\code{U} & 0.151 \\
\code{U9D} & 0.150 \\
\code{12U} & 0.150 \\
\code{10U} & 0.149 \\
\code{U8D} & 0.148 \\
\code{<self>} & 0.148 \\
\code{15U4D} & 0.148 \\
\code{U12D} & 0.148 \\
    \hline
    \end{tabular}
    \caption{Top UD paths ranked by the score aggregated from all attention heads in our trained \TreeRel model. See \secref{sec:learned-tree-rel} for more explanation.}
    \label{tab:top-aggr-ud-paths}
\end{table}



==> tab/top-eth-paths.tex <==
% This is a generated file. Do not manually modify. See <filename>.py instead.
\begin{table}[]
    \centering
    \begin{tabular}{l | r}
    \hline
    Equivalent $\mathit{UDpath}$ & Count \\
    \hline
    $U^1$ & $1.8 \times 10^{7}$ \\
$U^2D^1$ & $4.7 \times 10^{6}$ \\
$U^3$ & $4.2 \times 10^{6}$ \\
$U^2$ & $3.4 \times 10^{6}$ \\
$U^4$ & $3.0 \times 10^{6}$ \\
$U^2D^2$ & $2.9 \times 10^{6}$ \\
    \hline
    \end{tabular}
    \caption{Top $\mathit{UDpath}$-convertible tree-walks used by E13 when predicting values over py150.}
    \label{tab:top-eth-paths}
\end{table}



==> tab/top-ud-paths.tex <==
% This is a generated file. Do not manually modify. See <filename>.py instead.
\begin{table}[]
    \centering
    \begin{tabular}{l | r}
    \hline
    UD path & Count \\
    \hline
    \code{<self>} & 12 \\
\code{U} & 4 \\
\code{2U} & 3 \\
\code{UD} & 2 \\
\code{12U} & 2 \\
\code{U13D} & 2 \\
\code{U7D} & 1 \\
\code{3U} & 1 \\
\code{12U11D} & 1 \\
\code{16UD} & 1 \\
    \hline
    \end{tabular}
    \caption{Top UD relations ranked by the times of it being ranked as the top by the attention heads in out trained \TreeRel model.}
    \label{tab:top-ud-paths}
\end{table}


